Training Lightweight CNNs for Human-Nanodrone Proximity Interaction from Small Datasets using Background Randomization

We consider the task of visually estimating the pose of a human from images acquired by a nearby nano-drone; in this context, we propose a data augmentation approach based on synthetic background substitution to learn a lightweight CNN model from a small real-world training set. Experimental results on data from two different labs proves that the approach improves generalization to unseen environments.

==> sources/OLD_02-Related_work.tex <==
\section{Related Work}\label{sec:related_work}

The use of deep learning based methodologies for solving the task of autonomous control of unmanned aerial vehicle (UAV) has become the de-facto standard approach for solving such task.
Nonetheless, deep learning approaches still show major limitations. One of the most important one is the difficulty of these models, mainly neural networks, to generalize well from the training set.

One of the most common approaches tackling this impediment and improve neural networks' generalization capabilities is data augmentation; image augmentation when applied only on images.  
% When data augmentation is applied to images, thus the data augmentation that is utilised is Image augmentation.

Various approaches have been proposed for augmenting image based datasets~\cite{shorten2019augmentationsurvey}. The most common solutions apply geometric transformations~\cite{xie2020unsupervised} or erase parts of the images 
% to make sure that the model actually looks at the entire image while learning its task
~\cite{wan2013dropconn,zhong2017random}. Other methods combine multiple samples to create a new image. In~\cite{Takahashi_2020} and~\cite{summers2019improved}, augmented images are created as a collage of other randomly transformed samples. In~\cite{Lemley_2017}, the authors augment the dataset by creating a combination of images from the same classification category
% ; the result is similar to the intermediate outputs obtained during the application of a morphing effect \cite{wiki_morphing}
. More recently, machine learning approaches have been proposed for automatically learning image augmentation strategies~\cite{zoph2019learning, cubuk2019autoaugment}. 

An alternative to Image Augmentation is Domain Randomization. This technique is used to transfer a learned task from one domain into another. This method is useful when the real-world data is not easy to access and collect~\cite{mehta2019active}. Domain Randomization works by using data collected from a realistic simulation for training the model. The approach is used for reinforcement learning~\cite{imitation_learning_3d_navigation} and object recognition~\cite{weng2019DR, tobin2017domain}.
% Cite scaramuzza paper on domain randomization fro sim-to-real drone racing \cite{loquercio2019deep}
Recent studies have combined Domain Randomization and Image Augmentation. In \cite{yue2019domain}, the authors propose an interesting approach for augmenting a dataset using artistic style transfer \cite{gatys2015neural}.

We propose and test an approach for solving the problem of model generalization using synthetic domain randomization starting from the original work from Dario Mantegazza et al.~\cite{mantegazza2019visionbased}. The authors propose a machine learning model with the goal of continuously flying a drone in front of the moving user using images coming from the drone's front-facing camera. 
This papers is a fitting example of model generalization as the task is solved inside the room where the train data has been recorded, while it fails to replicate the results in other environments.
We compare the original network architecture and dataset defined in \cite{mantegazza2019visionbased} with a model trained on our augmented dataset.

% ----------- NANO-DRONE STUFF ----------- 

When autonomous navigation capabilities come to the nano-size class of UAVs, there are three main categories of solutions: \textit{i}) offloading the computation to some external power-unconstrained base-station~\cite{kang2019generalization,distance2018}; \textit{ii}) reducing the onboard workload's complexity to minimal functionalities~\cite{lowlevelcontrol2019,swarm2019}; \textit{iii}) extending the onboard brain either with general-purpose visual navigation engines~\cite{pulp-dronet1,pulp-dronet2,5liber,pulp-frontnet} based on the ULP heterogeneous model~\cite{ULP-hetero} or with application-specific processors~\cite{navion2019,slam2020}.
